The shortest confidence interval for the weighted sum of two Binomial proportions

Interval estimation of the probability of success in a Binomial model is considered. Zieli\'nski (2018) showed that the confidence interval which uses information about non-homogeneity of the sample is better than the classical one. In the following paper the shortest confidence interval for non-homogenous sample is constructed.

==> Fig_bin_krotkie.tex <==
%vartheta	pokrycie_kr
0.001	0.9992407
0.002	0.998729424
0.003	0.99706002
0.004	0.999118484
0.005	0.998326842
0.006	0.99719053
0.007	0.995665124
0.008	0.996241778
0.009	0.994717213
0.01	0.993560298
0.011	0.995408894
0.012	0.994022338
0.013	0.993699002
0.014	0.992161488
0.015	0.995529645
0.016	0.994356709
0.017	0.992988206
0.018	0.991409612
0.019	0.993736424
0.02	0.992446224
0.021	0.990983891
0.022	0.990771929
0.023	0.992924597
0.024	0.991666458
0.025	0.990258489
0.026	0.989367913
0.027	0.990058163
0.028	0.99288252
0.029	0.991737343
0.03	0.990465954
0.031	0.989061209
0.032	0.98894847
0.033	0.990744093
0.034	0.989465775
0.035	0.988065095
0.036	0.98904319
0.037	0.987703249
0.038	0.989847802
0.039	0.988592185
0.04	0.988219107
0.041	0.989160534
0.042	0.987930999
0.043	0.990186489
0.044	0.989027045
0.045	0.987769706
0.046	0.986999294
0.047	0.987341567
0.048	0.98900582
0.049	0.987827898
0.05	0.986559264
0.051	0.986135773
0.052	0.986863588
0.053	0.988569905
0.054	0.938154811
0.055	0.939625585
0.056	0.942627327
0.057	0.943813428
0.058	0.947233595
0.059	0.948176164
0.06	0.952087374
0.061	0.952827713
0.062	0.954214418
0.063	0.956503009
0.064	0.959553749
0.065	0.959980483
0.066	0.960249124
0.067	0.961898212
0.068	0.963997984
0.069	0.964096085
0.07	0.966697382
0.071	0.966675996
0.072	0.966524759
0.073	0.936816919
0.074	0.938075718
0.075	0.941449064
0.076	0.94501239
0.077	0.94601096
0.078	0.946843437
0.079	0.948916083
0.08	0.951387793
0.081	0.951981911
0.082	0.954880355
0.083	0.955314488
0.084	0.956186595
0.085	0.934104286
0.086	0.937211608
0.087	0.938278025
0.088	0.941548994
0.089	0.942422821
0.09	0.944287825
0.091	0.946535263
0.092	0.949200584
0.093	0.949802422
0.094	0.952471475
0.095	0.95291807
0.096	0.935400939
0.097	0.937646301
0.098	0.9404397
0.099	0.941370307
0.1	0.944345517
0.101	0.945999737
0.102	0.948023569
0.103	0.950440198
0.104	0.952924074
0.105	0.937047252
0.106	0.938466933
0.107	0.940353401
0.108	0.942721083
0.109	0.943565877
0.11	0.946124266
0.111	0.948741601
0.112	0.949398706
0.113	0.950528659
0.114	0.938157287
0.115	0.940791326
0.116	0.941759337
0.117	0.944431799
0.118	0.945233793
0.119	0.9470205
0.12	0.948986697
0.121	0.937764481
0.122	0.940348143
0.123	0.942988804
0.124	0.943805002
0.125	0.944994342
0.126	0.946659923
0.127	0.948700541
0.128	0.938555029
0.129	0.941073341
0.13	0.943665587
0.131	0.944421213
0.132	0.945791292
0.133	0.947615959
0.134	0.948162869
0.135	0.94053624
0.136	0.943068152
0.137	0.943846591
0.138	0.944936443
0.139	0.946481587
0.14	0.939262736
0.141	0.941626671
0.142	0.942390451
0.143	0.944780082
0.144	0.945410723
0.145	0.946579537
0.146	0.939629558
0.147	0.941820777
0.148	0.942513466
0.149	0.944738261
0.15	0.947069448
0.151	0.947608533
0.152	0.940974275
0.153	0.942903885
0.154	0.943510501
0.155	0.945564361
0.156	0.947684276
0.157	0.941657736
0.158	0.942848365
0.159	0.944469918
0.16	0.94637062
0.161	0.941611521
0.162	0.942292823
0.163	0.94455743
0.164	0.94512067
0.165	0.946353059
0.166	0.941494129
0.167	0.943514952
0.168	0.944092864
0.169	0.94612804
0.17	0.948324281
0.171	0.9424289
0.172	0.943926555
0.173	0.944436653
0.174	0.946189971
0.175	0.942884229
0.176	0.943464719
0.177	0.945593436
0.178	0.946721752
0.179	0.942662922
0.18	0.943221669
0.181	0.945064896
0.182	0.946955272
0.183	0.941745566
0.184	0.943930696
0.185	0.944400941
0.186	0.940752671
0.187	0.942508286
0.188	0.944369911
0.189	0.946291358
0.19	0.941588319
0.191	0.943854727
0.192	0.944342706
0.193	0.945783756
0.194	0.943532317
0.195	0.944045578
0.196	0.945888065
0.197	0.943241059
0.198	0.943767575
0.199	0.944992133
0.2	0.946530263
0.201	0.943474219
0.202	0.94394465
0.203	0.94575361
0.204	0.94208931
0.205	0.944236891
0.206	0.94465712
0.207	0.945970373
0.208	0.94320753
0.209	0.944936301
0.21	0.946766257
0.211	0.942650769
0.212	0.944830098
0.213	0.942302831
0.214	0.94383835
0.215	0.944258699
0.216	0.942169467
0.217	0.943960818
0.218	0.944361329
0.219	0.94633297
0.22	0.943626297
0.221	0.944015311
0.222	0.942226337
0.223	0.943917037
0.224	0.945675585
0.225	0.946021351
0.226	0.944378173
0.227	0.944754124
0.228	0.946077477
0.229	0.943762002
0.23	0.945373506
0.231	0.943440987
0.232	0.945302873
0.233	0.942419561
0.234	0.944617483
0.235	0.944980985
0.236	0.942904224
0.237	0.944514027
0.238	0.946154958
0.239	0.942847049
0.24	0.944824588
0.241	0.942569123
0.242	0.943872979
0.243	0.94535856
0.244	0.943788487
0.245	0.944136265
0.246	0.945835633
0.247	0.942839451
0.248	0.944892021
0.249	0.943477246
0.25	0.944847577
0.251	0.943639243
0.252	0.945203095
0.253	0.945496279
0.254	0.944293155
0.255	0.944593069
0.256	0.943485883
0.257	0.943802024
0.258	0.943046529
0.259	0.944573554
0.26	0.946169549
0.261	0.943736228
0.262	0.945698637
0.263	0.943003879
0.264	0.944292595
0.265	0.94570729
0.266	0.94408101
0.267	0.943102149
0.268	0.944835351
0.269	0.942862967
0.27	0.944920336
0.271	0.94518458
0.272	0.943925212
0.273	0.945356059
0.274	0.944040408
0.275	0.944304302
0.276	0.944389626
0.277	0.944653226
0.278	0.944350556
0.279	0.944620713
0.28	0.943361802
0.281	0.944795647
0.282	0.946367468
0.283	0.943880136
0.284	0.944864436
0.285	0.945127583
0.286	0.944464084
0.287	0.945848746
0.288	0.94374381
0.289	0.94512237
0.29	0.944301345
0.291	0.94454527
0.292	0.946512737
0.293	0.944138793
0.294	0.944069259
0.295	0.945438456
0.296	0.943656683
0.297	0.945113973
0.298	0.94466802
0.299	0.944899818
0.3	0.943712432
0.301	0.944903056
0.302	0.944391436
0.303	0.945841727
0.304	0.943803493
0.305	0.945578568
0.306	0.943318129
0.307	0.944440558
0.308	0.945612875
0.309	0.944314594
0.31	0.944683505
0.311	0.944795845
0.312	0.944729302
0.313	0.944839867
0.314	0.943816658
0.315	0.945001077
0.316	0.94629865
0.317	0.944076409
0.318	0.945758721
0.319	0.945808275
0.32	0.944724104
0.321	0.943391183
0.322	0.944580328
0.323	0.943863389
0.324	0.945383274
0.325	0.943342996
0.326	0.945136091
0.327	0.945202055
0.328	0.94410006
0.329	0.944322937
0.33	0.945443685
0.331	0.94546386
0.332	0.945541066
0.333	0.945371651
0.334	0.945444133
0.335	0.944460529
0.336	0.945599851
0.337	0.946950231
0.338	0.944451833
0.339	0.944963551
0.34	0.945039765
0.341	0.945118248
0.342	0.945186856
0.343	0.944397978
0.344	0.945527548
0.345	0.945006355
0.346	0.945070833
0.347	0.946825658
0.348	0.9440471
0.349	0.945180361
0.35	0.944979484
0.351	0.944330895
0.352	0.946000902
0.353	0.946062592
0.354	0.945898474
0.355	0.945953944
0.356	0.944805134
0.357	0.944921293
0.358	0.946390387
0.359	0.944957699
0.36	0.946693865
0.361	0.944981648
0.362	0.946710405
0.363	0.944844028
0.364	0.94599263
0.365	0.94706697
0.366	0.944568406
0.367	0.945028331
0.368	0.945072538
0.369	0.945297777
0.37	0.945334675
0.371	0.944686578
0.372	0.945818046
0.373	0.944770486
0.374	0.946475333
0.375	0.946495141
0.376	0.945541577
0.377	0.944281301
0.378	0.94543633
0.379	0.944939768
0.38	0.946503567
0.381	0.94478631
0.382	0.946549344
0.383	0.946575008
0.384	0.94603131
0.385	0.945060191
0.386	0.944791089
0.387	0.94588965
0.388	0.944257672
0.389	0.945986351
0.39	0.944083023
0.391	0.945894925
0.392	0.945904343
0.393	0.944595461
0.394	0.944563102
0.395	0.945610416
0.396	0.945880377
0.397	0.945920131
0.398	0.945993687
0.399	0.94602326
0.4	0.945068193
0.401	0.946165065
0.402	0.947789972
0.403	0.945276736
0.404	0.945297899
0.405	0.945868214
0.406	0.94438912
0.407	0.946100231
0.408	0.944378547
0.409	0.945539351
0.41	0.946588731
0.411	0.946172926
0.412	0.945185056
0.413	0.945639661
0.414	0.945677899
0.415	0.945308607
0.416	0.946440017
0.417	0.945536752
0.418	0.945549811
0.419	0.947337268
0.42	0.945004975
0.421	0.945608027
0.422	0.945627224
0.423	0.945396132
0.424	0.946478098
0.425	0.946611277
0.426	0.946623673
0.427	0.946388948
0.428	0.946414309
0.429	0.946389584
0.43	0.945695935
0.431	0.945663514
0.432	0.945670098
0.433	0.945329259
0.434	0.947174078
0.435	0.945469835
0.436	0.947274151
0.437	0.945152385
0.438	0.945342537
0.439	0.946486684
0.44	0.94620969
0.441	0.944758457
0.442	0.946617504
0.443	0.94660221
0.444	0.946454135
0.445	0.946442786
0.446	0.945378594
0.447	0.947153884
0.448	0.947207567
0.449	0.947694281
0.45	0.947737719
0.451	0.947754147
0.452	0.947789945
0.453	0.946959537
0.454	0.948010083
0.455	0.948013382
0.456	0.947649177
0.457	0.946530426
0.458	0.948319603
0.459	0.947029412
0.46	0.948231402
0.461	0.947667626
0.462	0.947677818
0.463	0.946614894
0.464	0.947478919
0.465	0.947513109
0.466	0.947976529
0.467	0.946640827
0.468	0.947830048
0.469	0.947047308
0.47	0.947063154
0.471	0.948949005
0.472	0.946853836
0.473	0.947628972
0.474	0.947656786
0.475	0.948008075
0.476	0.946419792
0.477	0.94761375
0.478	0.948641344
0.479	0.94672128
0.48	0.948664454
0.481	0.946558126
0.482	0.948365228
0.483	0.947273589
0.484	0.947253476
0.485	0.948398763
0.486	0.946713426
0.487	0.947685475
0.488	0.947609016
0.489	0.946649055
0.49	0.948337647
0.491	0.947177033
0.492	0.947097719
0.493	0.947097466
0.494	0.946354561
0.495	0.948357478
0.496	0.948354918
0.497	0.948210011
0.498	0.94718054
0.499	0.947176812
0.5	0.947575653
0.501	0.947176812
0.502	0.94718054
0.503	0.948210011
0.504	0.948354918
0.505	0.948357478
0.506	0.946354561
0.507	0.947097466
0.508	0.947097719
0.509	0.947177033
0.51	0.948337647
0.511	0.946649055
0.512	0.947609016
0.513	0.947685475
0.514	0.946713426
0.515	0.948398763
0.516	0.947253476
0.517	0.947273589
0.518	0.948365228
0.519	0.946558126
0.52	0.948664454
0.521	0.94672128
0.522	0.948641344
0.523	0.94761375
0.524	0.946419792
0.525	0.948008075
0.526	0.947656786
0.527	0.947628972
0.528	0.946853836
0.529	0.948949005
0.53	0.947063154
0.531	0.947047308
0.532	0.947830048
0.533	0.946640827
0.534	0.947976529
0.535	0.947513109
0.536	0.947478919
0.537	0.946614894
0.538	0.947677818
0.539	0.947667626
0.54	0.948231402
0.541	0.947029412
0.542	0.948319603
0.543	0.946530426
0.544	0.947649177
0.545	0.948013382
0.546	0.948010083
0.547	0.946959537
0.548	0.947789945
0.549	0.947754147
0.55	0.947737719
0.551	0.947694281
0.552	0.947207567
0.553	0.947153884
0.554	0.945378594
0.555	0.946442786
0.556	0.946454135
0.557	0.94660221
0.558	0.946617504
0.559	0.944758457
0.56	0.94620969
0.561	0.946486684
0.562	0.945342537
0.563	0.945152385
0.564	0.947274151
0.565	0.945469835
0.566	0.947174078
0.567	0.945329259
0.568	0.945670098
0.569	0.945663514
0.57	0.945695935
0.571	0.946389584
0.572	0.946414309
0.573	0.946388948
0.574	0.946623673
0.575	0.946611277
0.576	0.946478098
0.577	0.945396132
0.578	0.945627224
0.579	0.945608027
0.58	0.945004975
0.581	0.947337268
0.582	0.945549811
0.583	0.945536752
0.584	0.946440017
0.585	0.945308607
0.586	0.945677899
0.587	0.945639661
0.588	0.945185056
0.589	0.946172926
0.59	0.946588731
0.591	0.945539351
0.592	0.944378547
0.593	0.946100231
0.594	0.94438912
0.595	0.945868214
0.596	0.945297899
0.597	0.945276736
0.598	0.947789972
0.599	0.946165065
0.6	0.945068193
0.601	0.94602326
0.602	0.945993687
0.603	0.945920131
0.604	0.945880377
0.605	0.945610416
0.606	0.944563102
0.607	0.944595461
0.608	0.945904343
0.609	0.945894925
0.61	0.944083023
0.611	0.945986351
0.612	0.944257672
0.613	0.94588965
0.614	0.944791089
0.615	0.945060191
0.616	0.94603131
0.617	0.946575008
0.618	0.946549344
0.619	0.94478631
0.62	0.946503567
0.621	0.944939768
0.622	0.94543633
0.623	0.944281301
0.624	0.945541577
0.625	0.946495141
0.626	0.946475333
0.627	0.944770486
0.628	0.945818046
0.629	0.944686578
0.63	0.945334675
0.631	0.945297777
0.632	0.945072538
0.633	0.945028331
0.634	0.944568406
0.635	0.94706697
0.636	0.94599263
0.637	0.944844028
0.638	0.946710405
0.639	0.944981648
0.64	0.946693865
0.641	0.944957699
0.642	0.946390387
0.643	0.944921293
0.644	0.944805134
0.645	0.945953944
0.646	0.945898474
0.647	0.946062592
0.648	0.946000902
0.649	0.944330895
0.65	0.944979484
0.651	0.945180361
0.652	0.9440471
0.653	0.946825658
0.654	0.945070833
0.655	0.945006355
0.656	0.945527548
0.657	0.944397978
0.658	0.945186856
0.659	0.945118248
0.66	0.945039765
0.661	0.944963551
0.662	0.944451833
0.663	0.946950231
0.664	0.945599851
0.665	0.944460529
0.666	0.945444133
0.667	0.945371651
0.668	0.945541066
0.669	0.94546386
0.67	0.945443685
0.671	0.944322937
0.672	0.94410006
0.673	0.945202055
0.674	0.945136091
0.675	0.943342996
0.676	0.945383274
0.677	0.943863389
0.678	0.944580328
0.679	0.943391183
0.68	0.944724104
0.681	0.945808275
0.682	0.945758721
0.683	0.944076409
0.684	0.94629865
0.685	0.945001077
0.686	0.943816658
0.687	0.944839867
0.688	0.944729302
0.689	0.944795845
0.69	0.944683505
0.691	0.944314594
0.692	0.945612875
0.693	0.944440558
0.694	0.943318129
0.695	0.945578568
0.696	0.943803493
0.697	0.945841727
0.698	0.944391436
0.699	0.944903056
0.7	0.944467112
0.701	0.944899818
0.702	0.94466802
0.703	0.945113973
0.704	0.943656683
0.705	0.945438456
0.706	0.944069259
0.707	0.944138793
0.708	0.946512737
0.709	0.94454527
0.71	0.944301345
0.711	0.94512237
0.712	0.94374381
0.713	0.945848746
0.714	0.944464084
0.715	0.945127583
0.716	0.944864436
0.717	0.943880136
0.718	0.946367468
0.719	0.944795647
0.72	0.943361802
0.721	0.944620713
0.722	0.944350556
0.723	0.944653226
0.724	0.944389626
0.725	0.944304302
0.726	0.944040408
0.727	0.945356059
0.728	0.943925212
0.729	0.94518458
0.73	0.944920336
0.731	0.942862967
0.732	0.944835351
0.733	0.943102149
0.734	0.94408101
0.735	0.94570729
0.736	0.944292595
0.737	0.943003879
0.738	0.945698637
0.739	0.943736228
0.74	0.946169549
0.741	0.944573554
0.742	0.943046529
0.743	0.943802024
0.744	0.943485883
0.745	0.944593069
0.746	0.944293155
0.747	0.945496279
0.748	0.945203095
0.749	0.943639243
0.75	0.944847577
0.751	0.943477246
0.752	0.944892021
0.753	0.942839451
0.754	0.945835633
0.755	0.944136265
0.756	0.943788487
0.757	0.94535856
0.758	0.943872979
0.759	0.942569123
0.76	0.944824588
0.761	0.942847049
0.762	0.946154958
0.763	0.944514027
0.764	0.942904224
0.765	0.944980985
0.766	0.944617483
0.767	0.942419561
0.768	0.945302873
0.769	0.943440987
0.77	0.945373506
0.771	0.943762002
0.772	0.946077477
0.773	0.944754124
0.774	0.944378173
0.775	0.946021351
0.776	0.945675585
0.777	0.943917037
0.778	0.942226337
0.779	0.944015311
0.78	0.943626297
0.781	0.94633297
0.782	0.944361329
0.783	0.943960818
0.784	0.942169467
0.785	0.944258699
0.786	0.94383835
0.787	0.942302831
0.788	0.944830098
0.789	0.942650769
0.79	0.946766257
0.791	0.944936301
0.792	0.94320753
0.793	0.945970373
0.794	0.94465712
0.795	0.944236891
0.796	0.94208931
0.797	0.94575361
0.798	0.94394465
0.799	0.943474219
0.8	0.946530263
0.801	0.944992133
0.802	0.943767575
0.803	0.943241059
0.804	0.945888065
0.805	0.944045578
0.806	0.943532317
0.807	0.945783756
0.808	0.944342706
0.809	0.943854727
0.81	0.941588319
0.811	0.946291358
0.812	0.944369911
0.813	0.942508286
0.814	0.940752671
0.815	0.944400941
0.816	0.943930696
0.817	0.941745566
0.818	0.946955272
0.819	0.945064896
0.82	0.943221669
0.821	0.942662922
0.822	0.946721752
0.823	0.945593436
0.824	0.943464719
0.825	0.942884229
0.826	0.946189971
0.827	0.944436653
0.828	0.943926555
0.829	0.9424289
0.83	0.948324281
0.831	0.94612804
0.832	0.944092864
0.833	0.943514952
0.834	0.941494129
0.835	0.946353059
0.836	0.94512067
0.837	0.94455743
0.838	0.942292823
0.839	0.941611521
0.84	0.94637062
0.841	0.944469918
0.842	0.942848365
0.843	0.941657736
0.844	0.947684276
0.845	0.945564361
0.846	0.943510501
0.847	0.942903885
0.848	0.940974275
0.849	0.947608533
0.85	0.947069448
0.851	0.944738261
0.852	0.942513466
0.853	0.941820777
0.854	0.939629558
0.855	0.946579537
0.856	0.945410723
0.857	0.944780082
0.858	0.942390451
0.859	0.941626671
0.86	0.939262736
0.861	0.946481587
0.862	0.944936443
0.863	0.943846591
0.864	0.943068152
0.865	0.94053624
0.866	0.948162869
0.867	0.947615959
0.868	0.945791292
0.869	0.944421213
0.87	0.943665587
0.871	0.941073341
0.872	0.938555029
0.873	0.948700541
0.874	0.946659923
0.875	0.944994342
0.876	0.943805002
0.877	0.942988804
0.878	0.940348143
0.879	0.937764481
0.88	0.948986697
0.881	0.9470205
0.882	0.945233793
0.883	0.944431799
0.884	0.941759337
0.885	0.940791326
0.886	0.938157287
0.887	0.950528659
0.888	0.949398706
0.889	0.948741601
0.89	0.946124266
0.891	0.943565877
0.892	0.942721083
0.893	0.940353401
0.894	0.938466933
0.895	0.937047252
0.896	0.952924074
0.897	0.950440198
0.898	0.948023569
0.899	0.945999737
0.9	0.944345517
0.901	0.941370307
0.902	0.9404397
0.903	0.937646301
0.904	0.935400939
0.905	0.95291807
0.906	0.952471475
0.907	0.949802422
0.908	0.949200584
0.909	0.946535263
0.91	0.944287825
0.911	0.942422821
0.912	0.941548994
0.913	0.938278025
0.914	0.937211608
0.915	0.934104286
0.916	0.956186595
0.917	0.955314488
0.918	0.954880355
0.919	0.951981911
0.92	0.951387793
0.921	0.948916083
0.922	0.946843437
0.923	0.94601096
0.924	0.94501239
0.925	0.941449064
0.926	0.938075718
0.927	0.936816919
0.928	0.966524759
0.929	0.966675996
0.93	0.966697382
0.931	0.964096085
0.932	0.963997984
0.933	0.961898212
0.934	0.960249124
0.935	0.959980483
0.936	0.959553749
0.937	0.956503009
0.938	0.954214418
0.939	0.952827713
0.94	0.952087374
0.941	0.948176164
0.942	0.947233595
0.943	0.943813428
0.944	0.942627327
0.945	0.939625585
0.946	0.938154811
0.947	0.988569905
0.948	0.986863588
0.949	0.986135773
0.95	0.986559264
0.951	0.987827898
0.952	0.98900582
0.953	0.987341567
0.954	0.986999294
0.955	0.987769706
0.956	0.989027045
0.957	0.990186489
0.958	0.987930999
0.959	0.989160534
0.96	0.988219107
0.961	0.988592185
0.962	0.989847802
0.963	0.987703249
0.964	0.98904319
0.965	0.988065095
0.966	0.989465775
0.967	0.990744093
0.968	0.98894847
0.969	0.989061209
0.97	0.990465954
0.971	0.991737343
0.972	0.99288252
0.973	0.990058163
0.974	0.989367913
0.975	0.990258489
0.976	0.991666458
0.977	0.992924597
0.978	0.990771929
0.979	0.990983891
0.98	0.992446224
0.981	0.993736424
0.982	0.991409612
0.983	0.992988206
0.984	0.994356709
0.985	0.995529645
0.986	0.992161488
0.987	0.993699002
0.988	0.994022338
0.989	0.995408894
0.99	0.993560298
0.991	0.994717213
0.992	0.996241778
0.993	0.995665124
0.994	0.99719053
0.995	0.998326842
0.996	0.999118484
0.997	0.99706002
0.998	0.998729424
0.999	0.9992407


==> Fig_bin_krotkie_rand.tex <==
%vartheta	pokrycie_kr
0.001	0.9994
0.002	0.9988
0.003	0.9973
0.004	0.9992
0.005	0.9987
0.006	0.998
0.007	0.9973
0.008	0.9963
0.009	0.9951
0.01	0.9963
0.011	0.9956
0.012	0.9947
0.013	0.9937
0.014	0.9961
0.015	0.9956
0.016	0.9946
0.017	0.9934
0.018	0.9921
0.019	0.9938
0.02	0.9929
0.021	0.9919
0.022	0.9927
0.023	0.993
0.024	0.9919
0.025	0.9907
0.026	0.9908
0.027	0.992
0.028	0.9929
0.029	0.992
0.03	0.9911
0.031	0.9902
0.032	0.991
0.033	0.9908
0.034	0.9898
0.035	0.9886
0.036	0.9896
0.037	0.9903
0.038	0.9901
0.039	0.9891
0.04	0.9882
0.041	0.9892
0.042	0.9899
0.043	0.9902
0.044	0.9892
0.045	0.9881
0.046	0.9876
0.047	0.9884
0.048	0.989
0.049	0.9881
0.05	0.9872
0.051	0.9877
0.052	0.9883
0.053	0.9886
0.054	0.9876
0.055	0.9865
0.056	0.9866
0.057	0.9831
0.058	0.9837
0.059	0.9806
0.06	0.9804
0.061	0.9814
0.062	0.9819
0.063	0.9801
0.064	0.9812
0.065	0.9782
0.066	0.9779
0.067	0.9762
0.068	0.9778
0.069	0.9768
0.07	0.9756
0.071	0.9756
0.072	0.9737
0.073	0.9736
0.074	0.9719
0.075	0.9733
0.076	0.9717
0.077	0.9691
0.078	0.9668
0.079	0.9684
0.08	0.9678
0.081	0.9672
0.082	0.9659
0.083	0.9643
0.084	0.9637
0.085	0.9638
0.086	0.9653
0.087	0.9647
0.088	0.9631
0.089	0.9615
0.09	0.9612
0.091	0.9611
0.092	0.961
0.093	0.9609
0.094	0.9605
0.095	0.9595
0.096	0.9589
0.097	0.9592
0.098	0.9592
0.099	0.9592
0.1	0.9584
0.101	0.9592
0.102	0.9595
0.103	0.9586
0.104	0.9589
0.105	0.9584
0.106	0.9575
0.107	0.9579
0.108	0.9582
0.109	0.9584
0.11	0.9586
0.111	0.9574
0.112	0.9569
0.113	0.9566
0.114	0.9572
0.115	0.9563
0.116	0.9566
0.117	0.9554
0.118	0.9549
0.119	0.954
0.12	0.9548
0.121	0.9543
0.122	0.9549
0.123	0.9554
0.124	0.9551
0.125	0.9538
0.126	0.9548
0.127	0.9545
0.128	0.9553
0.129	0.9547
0.13	0.9553
0.131	0.9543
0.132	0.9542
0.133	0.9541
0.134	0.955
0.135	0.9546
0.136	0.9543
0.137	0.9541
0.138	0.9533
0.139	0.9535
0.14	0.9536
0.141	0.9543
0.142	0.9541
0.143	0.9537
0.144	0.9537
0.145	0.9535
0.146	0.9538
0.147	0.9536
0.148	0.9534
0.149	0.9542
0.15	0.9541
0.151	0.9535
0.152	0.9531
0.153	0.9532
0.154	0.9531
0.155	0.9532
0.156	0.9532
0.157	0.9519
0.158	0.9518
0.159	0.9522
0.16	0.9527
0.161	0.9531
0.162	0.9532
0.163	0.9532
0.164	0.9528
0.165	0.9522
0.166	0.9526
0.167	0.9527
0.168	0.953
0.169	0.9533
0.17	0.9536
0.171	0.9527
0.172	0.9523
0.173	0.9526
0.174	0.9523
0.175	0.9527
0.176	0.9526
0.177	0.9525
0.178	0.9519
0.179	0.9525
0.18	0.9524
0.181	0.9527
0.182	0.9532
0.183	0.953
0.184	0.9522
0.185	0.9515
0.186	0.9515
0.187	0.9518
0.188	0.9518
0.189	0.9523
0.19	0.9525
0.191	0.9521
0.192	0.9516
0.193	0.9512
0.194	0.9514
0.195	0.952
0.196	0.9523
0.197	0.9526
0.198	0.9521
0.199	0.9517
0.2	0.9523
0.201	0.9524
0.202	0.9524
0.203	0.9518
0.204	0.9519
0.205	0.952
0.206	0.9517
0.207	0.952
0.208	0.9521
0.209	0.9522
0.21	0.9523
0.211	0.9524
0.212	0.9518
0.213	0.9506
0.214	0.9506
0.215	0.9512
0.216	0.9514
0.217	0.9517
0.218	0.9519
0.219	0.9518
0.22	0.9514
0.221	0.9513
0.222	0.9511
0.223	0.9515
0.224	0.9519
0.225	0.9524
0.226	0.9519
0.227	0.9517
0.228	0.9517
0.229	0.9515
0.23	0.9508
0.231	0.951
0.232	0.9514
0.233	0.9518
0.234	0.9518
0.235	0.9518
0.236	0.9517
0.237	0.9519
0.238	0.9522
0.239	0.9521
0.24	0.9515
0.241	0.9505
0.242	0.9508
0.243	0.951
0.244	0.9513
0.245	0.9517
0.246	0.9518
0.247	0.9517
0.248	0.9506
0.249	0.9503
0.25	0.9509
0.251	0.9514
0.252	0.9515
0.253	0.9521
0.254	0.9521
0.255	0.9521
0.256	0.9518
0.257	0.9511
0.258	0.9506
0.259	0.951
0.26	0.9514
0.261	0.9517
0.262	0.9516
0.263	0.9514
0.264	0.9515
0.265	0.9515
0.266	0.9509
0.267	0.9501
0.268	0.9507
0.269	0.9514
0.27	0.9513
0.271	0.9511
0.272	0.9511
0.273	0.9513
0.274	0.9515
0.275	0.9508
0.276	0.951
0.277	0.9513
0.278	0.9515
0.279	0.9514
0.28	0.9513
0.281	0.9513
0.282	0.9516
0.283	0.9507
0.284	0.9503
0.285	0.9506
0.286	0.9506
0.287	0.9511
0.288	0.9512
0.289	0.9516
0.29	0.9519
0.291	0.9517
0.292	0.9517
0.293	0.9504
0.294	0.9501
0.295	0.9505
0.296	0.951
0.297	0.9514
0.298	0.9516
0.299	0.9515
0.3	0.9514
0.301	0.9503
0.302	0.9509
0.303	0.9512
0.304	0.9515
0.305	0.9514
0.306	0.9512
0.307	0.9511
0.308	0.9512
0.309	0.9507
0.31	0.9507
0.311	0.951
0.312	0.9512
0.313	0.9511
0.314	0.9513
0.315	0.9512
0.316	0.9515
0.317	0.952
0.318	0.952
0.319	0.9523
0.32	0.9513
0.321	0.9503
0.322	0.9507
0.323	0.9512
0.324	0.9515
0.325	0.9517
0.326	0.9515
0.327	0.951
0.328	0.9501
0.329	0.9503
0.33	0.9511
0.331	0.9514
0.332	0.9517
0.333	0.9517
0.334	0.9514
0.335	0.9515
0.336	0.9518
0.337	0.9522
0.338	0.9512
0.339	0.951
0.34	0.9513
0.341	0.9513
0.342	0.9511
0.343	0.9514
0.344	0.9515
0.345	0.9519
0.346	0.9522
0.347	0.9522
0.348	0.9516
0.349	0.9507
0.35	0.9509
0.351	0.9512
0.352	0.9519
0.353	0.9519
0.354	0.952
0.355	0.9517
0.356	0.9512
0.357	0.9507
0.358	0.9513
0.359	0.9517
0.36	0.9519
0.361	0.9517
0.362	0.9518
0.363	0.9516
0.364	0.9517
0.365	0.952
0.366	0.9517
0.367	0.9512
0.368	0.9516
0.369	0.9515
0.37	0.9513
0.371	0.9515
0.372	0.9518
0.373	0.9523
0.374	0.9525
0.375	0.9528
0.376	0.9521
0.377	0.9511
0.378	0.9512
0.379	0.9515
0.38	0.952
0.381	0.9521
0.382	0.9523
0.383	0.9524
0.384	0.9512
0.385	0.951
0.386	0.9511
0.387	0.9515
0.388	0.952
0.389	0.9522
0.39	0.9523
0.391	0.9522
0.392	0.9522
0.393	0.9518
0.394	0.951
0.395	0.9516
0.396	0.9522
0.397	0.9521
0.398	0.9521
0.399	0.952
0.4	0.9522
0.401	0.9524
0.402	0.9531
0.403	0.9529
0.404	0.9518
0.405	0.9518
0.406	0.9518
0.407	0.9518
0.408	0.9517
0.409	0.9518
0.41	0.9525
0.411	0.9519
0.412	0.9517
0.413	0.9518
0.414	0.9516
0.415	0.9517
0.416	0.9518
0.417	0.9521
0.418	0.9528
0.419	0.9529
0.42	0.9525
0.421	0.9517
0.422	0.9516
0.423	0.9517
0.424	0.9521
0.425	0.9526
0.426	0.9529
0.427	0.9529
0.428	0.9529
0.429	0.9528
0.43	0.9521
0.431	0.9516
0.432	0.9516
0.433	0.9523
0.434	0.9527
0.435	0.9526
0.436	0.9527
0.437	0.9522
0.438	0.9513
0.439	0.9516
0.44	0.9518
0.441	0.9524
0.442	0.9527
0.443	0.9528
0.444	0.9528
0.445	0.9526
0.446	0.9524
0.447	0.9535
0.448	0.9536
0.449	0.9536
0.45	0.9538
0.451	0.9539
0.452	0.9536
0.453	0.9537
0.454	0.9537
0.455	0.9546
0.456	0.954
0.457	0.9534
0.458	0.9535
0.459	0.9534
0.46	0.9534
0.461	0.9537
0.462	0.9536
0.463	0.9538
0.464	0.9533
0.465	0.9536
0.466	0.9535
0.467	0.9534
0.468	0.9534
0.469	0.9538
0.47	0.9545
0.471	0.9545
0.472	0.9539
0.473	0.9535
0.474	0.9534
0.475	0.9536
0.476	0.9536
0.477	0.9536
0.478	0.9537
0.479	0.9545
0.48	0.9545
0.481	0.9544
0.482	0.9535
0.483	0.9533
0.484	0.9532
0.485	0.9535
0.486	0.9534
0.487	0.954
0.488	0.9542
0.489	0.9533
0.49	0.9533
0.491	0.9533
0.492	0.9533
0.493	0.9534
0.494	0.9543
0.495	0.9545
0.496	0.9545
0.497	0.9541
0.498	0.9534
0.499	0.9534
0.5	0.9534
0.501	0.9535
0.502	0.9534
0.503	0.9541
0.504	0.9545
0.505	0.9545
0.506	0.9543
0.507	0.9534
0.508	0.9533
0.509	0.9533
0.51	0.9534
0.511	0.9534
0.512	0.9542
0.513	0.954
0.514	0.9534
0.515	0.9535
0.516	0.9532
0.517	0.9533
0.518	0.9534
0.519	0.9544
0.52	0.9544
0.521	0.9545
0.522	0.9537
0.523	0.9535
0.524	0.9535
0.525	0.9536
0.526	0.9535
0.527	0.9536
0.528	0.9538
0.529	0.9545
0.53	0.9545
0.531	0.9538
0.532	0.9534
0.533	0.9534
0.534	0.9535
0.535	0.9536
0.536	0.9534
0.537	0.9538
0.538	0.9535
0.539	0.9536
0.54	0.9534
0.541	0.9533
0.542	0.9535
0.543	0.9534
0.544	0.9539
0.545	0.9546
0.546	0.9537
0.547	0.9536
0.548	0.9536
0.549	0.9538
0.55	0.9538
0.551	0.9536
0.552	0.9536
0.553	0.9535
0.554	0.9523
0.555	0.9526
0.556	0.9527
0.557	0.9529
0.558	0.9527
0.559	0.9524
0.56	0.9519
0.561	0.9516
0.562	0.9513
0.563	0.9521
0.564	0.9527
0.565	0.9526
0.566	0.9527
0.567	0.9523
0.568	0.9516
0.569	0.9515
0.57	0.952
0.571	0.9528
0.572	0.9529
0.573	0.9529
0.574	0.9529
0.575	0.9526
0.576	0.9522
0.577	0.9517
0.578	0.9516
0.579	0.9517
0.58	0.9524
0.581	0.9529
0.582	0.9528
0.583	0.9521
0.584	0.9518
0.585	0.9517
0.586	0.9516
0.587	0.9518
0.588	0.9518
0.589	0.9518
0.59	0.9525
0.591	0.9518
0.592	0.9516
0.593	0.9518
0.594	0.9518
0.595	0.9519
0.596	0.9518
0.597	0.9528
0.598	0.9531
0.599	0.9524
0.6	0.9521
0.601	0.952
0.602	0.9521
0.603	0.9521
0.604	0.9523
0.605	0.9517
0.606	0.951
0.607	0.9516
0.608	0.9521
0.609	0.9521
0.61	0.9523
0.611	0.9522
0.612	0.952
0.613	0.9515
0.614	0.9511
0.615	0.951
0.616	0.9511
0.617	0.9524
0.618	0.9523
0.619	0.9521
0.62	0.952
0.621	0.9515
0.622	0.9512
0.623	0.951
0.624	0.9519
0.625	0.9527
0.626	0.9525
0.627	0.9523
0.628	0.9517
0.629	0.9514
0.63	0.9513
0.631	0.9515
0.632	0.9516
0.633	0.9513
0.634	0.9516
0.635	0.9519
0.636	0.9516
0.637	0.9515
0.638	0.9517
0.639	0.9517
0.64	0.9519
0.641	0.9517
0.642	0.9514
0.643	0.9507
0.644	0.9511
0.645	0.9516
0.646	0.9519
0.647	0.9519
0.648	0.9519
0.649	0.9512
0.65	0.9509
0.651	0.9505
0.652	0.9514
0.653	0.9521
0.654	0.9521
0.655	0.9519
0.656	0.9515
0.657	0.9513
0.658	0.951
0.659	0.9513
0.66	0.9514
0.661	0.951
0.662	0.9511
0.663	0.9521
0.664	0.9517
0.665	0.9514
0.666	0.9513
0.667	0.9516
0.668	0.9518
0.669	0.9514
0.67	0.9512
0.671	0.9503
0.672	0.95
0.673	0.951
0.674	0.9514
0.675	0.9516
0.676	0.9515
0.677	0.9512
0.678	0.9507
0.679	0.9503
0.68	0.9511
0.681	0.9522
0.682	0.952
0.683	0.952
0.684	0.9515
0.685	0.9511
0.686	0.9512
0.687	0.951
0.688	0.9511
0.689	0.9511
0.69	0.9507
0.691	0.9506
0.692	0.9511
0.693	0.9509
0.694	0.951
0.695	0.9513
0.696	0.9515
0.697	0.9512
0.698	0.9509
0.699	0.9504
0.7	0.9513
0.701	0.9515
0.702	0.9515
0.703	0.9513
0.704	0.951
0.705	0.9505
0.706	0.95
0.707	0.9502
0.708	0.9515
0.709	0.9516
0.71	0.9518
0.711	0.9515
0.712	0.9511
0.713	0.951
0.714	0.9505
0.715	0.9506
0.716	0.9503
0.717	0.9506
0.718	0.9515
0.719	0.9512
0.72	0.9511
0.721	0.9512
0.722	0.9514
0.723	0.9513
0.724	0.951
0.725	0.9507
0.726	0.9514
0.727	0.9512
0.728	0.951
0.729	0.951
0.73	0.9512
0.731	0.9513
0.732	0.9507
0.733	0.9501
0.734	0.9507
0.735	0.9513
0.736	0.9513
0.737	0.9512
0.738	0.9515
0.739	0.9516
0.74	0.9514
0.741	0.951
0.742	0.9505
0.743	0.9509
0.744	0.9516
0.745	0.952
0.746	0.952
0.747	0.952
0.748	0.9514
0.749	0.9512
0.75	0.9508
0.751	0.9502
0.752	0.9504
0.753	0.9515
0.754	0.9517
0.755	0.9516
0.756	0.9511
0.757	0.9509
0.758	0.9506
0.759	0.9503
0.76	0.9512
0.761	0.9519
0.762	0.952
0.763	0.9517
0.764	0.9515
0.765	0.9516
0.766	0.9516
0.767	0.9516
0.768	0.9513
0.769	0.9509
0.77	0.9506
0.771	0.9512
0.772	0.9515
0.773	0.9514
0.774	0.9517
0.775	0.9522
0.776	0.9518
0.777	0.9513
0.778	0.9509
0.779	0.951
0.78	0.9512
0.781	0.9515
0.782	0.9517
0.783	0.9515
0.784	0.9512
0.785	0.951
0.786	0.9505
0.787	0.9504
0.788	0.9515
0.789	0.9521
0.79	0.9521
0.791	0.9519
0.792	0.9518
0.793	0.9518
0.794	0.9514
0.795	0.9517
0.796	0.9517
0.797	0.9515
0.798	0.952
0.799	0.9521
0.8	0.952
0.801	0.9513
0.802	0.9517
0.803	0.9522
0.804	0.9521
0.805	0.9517
0.806	0.9511
0.807	0.9509
0.808	0.9512
0.809	0.9517
0.81	0.9521
0.811	0.9521
0.812	0.9515
0.813	0.9515
0.814	0.9511
0.815	0.951
0.816	0.9518
0.817	0.9526
0.818	0.9528
0.819	0.9523
0.82	0.952
0.821	0.9521
0.822	0.9515
0.823	0.9521
0.824	0.9522
0.825	0.9523
0.826	0.9519
0.827	0.9521
0.828	0.9518
0.829	0.9521
0.83	0.9531
0.831	0.9528
0.832	0.9526
0.833	0.9523
0.834	0.9521
0.835	0.9517
0.836	0.9522
0.837	0.9526
0.838	0.9527
0.839	0.9526
0.84	0.9522
0.841	0.9518
0.842	0.9513
0.843	0.9513
0.844	0.9525
0.845	0.9527
0.846	0.9525
0.847	0.9525
0.848	0.9524
0.849	0.9529
0.85	0.9534
0.851	0.9536
0.852	0.9528
0.853	0.9529
0.854	0.953
0.855	0.9528
0.856	0.953
0.857	0.953
0.858	0.9534
0.859	0.9536
0.86	0.9528
0.861	0.9528
0.862	0.9526
0.863	0.9532
0.864	0.9534
0.865	0.9538
0.866	0.9543
0.867	0.9534
0.868	0.9534
0.869	0.9534
0.87	0.9544
0.871	0.9539
0.872	0.9544
0.873	0.9537
0.874	0.9539
0.875	0.9529
0.876	0.9541
0.877	0.9544
0.878	0.9539
0.879	0.9532
0.88	0.9539
0.881	0.953
0.882	0.9537
0.883	0.9542
0.884	0.9554
0.885	0.9551
0.886	0.956
0.887	0.9555
0.888	0.9557
0.889	0.9561
0.89	0.9574
0.891	0.9571
0.892	0.9569
0.893	0.9565
0.894	0.956
0.895	0.9568
0.896	0.9577
0.897	0.9574
0.898	0.9583
0.899	0.9578
0.9	0.9568
0.901	0.9578
0.902	0.9577
0.903	0.9576
0.904	0.9572
0.905	0.958
0.906	0.9589
0.907	0.9594
0.908	0.9595
0.909	0.9594
0.91	0.9594
0.911	0.9595
0.912	0.9611
0.913	0.9627
0.914	0.9633
0.915	0.9616
0.916	0.962
0.917	0.9624
0.918	0.9639
0.919	0.9653
0.92	0.9658
0.921	0.9662
0.922	0.9643
0.923	0.9666
0.924	0.969
0.925	0.9706
0.926	0.9691
0.927	0.9707
0.928	0.972
0.929	0.9737
0.93	0.9736
0.931	0.9749
0.932	0.9758
0.933	0.974
0.934	0.9754
0.935	0.9756
0.936	0.9784
0.937	0.9774
0.938	0.9789
0.939	0.9782
0.94	0.9818
0.941	0.982
0.942	0.9801
0.943	0.984
0.944	0.9824
0.945	0.9819
0.946	0.9827
0.947	0.9886
0.948	0.9885
0.949	0.9879
0.95	0.9873
0.951	0.9882
0.952	0.9891
0.953	0.9887
0.954	0.9878
0.955	0.9882
0.956	0.9893
0.957	0.9902
0.958	0.9903
0.959	0.9895
0.96	0.9884
0.961	0.9892
0.962	0.9902
0.963	0.9907
0.964	0.9899
0.965	0.9886
0.966	0.9898
0.967	0.9909
0.968	0.9913
0.969	0.9903
0.97	0.9912
0.971	0.9921
0.972	0.993
0.973	0.9924
0.974	0.991
0.975	0.9908
0.976	0.9919
0.977	0.993
0.978	0.9931
0.979	0.9921
0.98	0.993
0.981	0.9939
0.982	0.9922
0.983	0.9935
0.984	0.9947
0.985	0.9956
0.986	0.9965
0.987	0.9941
0.988	0.9948
0.989	0.9957
0.99	0.9966
0.991	0.9952
0.992	0.9964
0.993	0.9975
0.994	0.9981
0.995	0.9988
0.996	0.9992
0.997	0.9973
0.998	0.9988
0.999	0.9995

